Predicting Audio Advertisement Quality

Online audio advertising is a particular form of advertising used abundantly in online music streaming services. In these platforms, which tend to host tens of thousands of unique audio advertisements (ads), providing high quality ads ensures a better user experience and results in longer user engagement. Therefore, the automatic assessment of these ads is an important step toward audio ads ranking and better audio ads creation. In this paper we propose one way to measure the quality of the audio ads using a proxy metric called Long Click Rate (LCR), which is defined by the amount of time a user engages with the follow-up display ad (that is shown while the audio ad is playing) divided by the impressions. We later focus on predicting the audio ad quality using only acoustic features such as harmony, rhythm, and timbre of the audio, extracted from the raw waveform. We discuss how the characteristics of the sound can be connected to concepts such as the clarity of the audio ad message, its trustworthiness, etc. Finally, we propose a new deep learning model for audio ad quality prediction, which outperforms the other discussed models trained on hand-crafted features. To the best of our knowledge, this is the first large-scale audio ad quality prediction study.

==> body.tex <==
%!TEX root = paper.tex
%

\section{Related work}
Click Prediction ...


There are several works in the literature focusing on Predicting the CTR ,~\cite{chakrabarti2008contextual} proposed a model that combines click feedback and contextual advertising system using logistic regression. ~\cite{cheng2010personalized} developed user-specific and demographic based features for click prediction in sponsored search. ~\cite{dave2010learning} used decision trees for click prediction
to Predict CTR for new ads.

\textbf{edit}"Since the display advertising has taken a large share of online advertising market, many works addressing the CTR prediction problem have been published. In ~\cite{richardson2007predicting}, ~\cite{chakrabarti2008contextual}, authors handcraft many features from raw data and use logistic regression (LR) to predict the click-through rate. ~\cite{chapelle2015simple} also uses LR to deal with the CTR problem and scales it to billions of samples and millions of parameters on a distributed learning system. In ~\cite{oentaryo2014predicting}, a Hierarchical Importance-aware Factorization Machine (FM) is introduced, which provides a generic latent factor framework that incorporates importance weights and hierarchical learning. In ~\cite{dave2010learning}, boosted decision trees have been used to build a prediction model. In ~\cite{he2014practical}, a model which combines decision trees with logistic regression has been proposed, and outperforms either of the above two models. ~\cite{zhang2016deep} combines deep neural networks with FM and also brings an improvement. All of these methods are very effective when deal with ads without images. However, when it comes to the image ads, they can only use pre-extracted image features, which is less flexible to take account of the unique properties of different datasets. 
"
\textbf{edit(display ad)}"The image features in display advertisement have received more and more attention. In ~\cite{azimi2012impact}, ~\cite{cheng2012multimedia}, the impact of visual appearance on user’s response in online display advertising is considered for the first time. They extract over 30 handcrafted features from ad images and build a CTR prediction model using image and basic features. The experiment result shows that their method achieves better performance than models without visual features. ~\cite{mo2015image} is the most related work in literature with us, in which a decapitated convolutional neural network (CNN) is used to extract image features from ads. "

~\cite{chen2016deep} "proposed a deep neural network (DNN) based model that directly predicts the CTR of an image ad based on raw image pixels and other basic features in one step. The DNN model use convolution layers to automatically extract representative visual features from images, and nonlinear CTR features are then learned from visual features and other contextual features by using fully-connected layers. "
~\cite{zhou2016predicting} "\textbf{We presented} an approach that aimed at identifying low quality ads, from the pre-click experience. Our focus was native advertising, where the ads served reproduce the look- and-feel of the platform in which they appear. As our proxy of low pre-click quality, we used the ad offensiveness anno- tations extracted from an ad feedback mechanism used by a large Internet company. We showed that ad offensive- ness feedback rate, which we use as our learning target, is different to CTR, and that it is important to deploy compu- tational approaches to detect offensive ads, independently of whether they are clicked or not."


\textbf{edit}"The majority of current models use logistic regression based on a set of sparse binary features converted from the original categorical features via one-hot encoding [~\cite{lee2012estimating},~\cite{richardson2007predicting}]. Heavy engineering efforts are needed to design features such as locations, top unigrams, combination features, etc. [~\cite{he2014practical}]. 
"
Many work in the literature addressed the cold start problem for predicting new ads, 

Most of the focus in the literature is on predicting the quality of display ads, and to the best of our knowledge there is no work until now using audio ads' features itself to predict the audio ad quality.


In order to predict CTR of new ads, many works addressed the cold start problem in various ways. Chakrabarti [Chakrabarti et al., 2008] used contextual information while Kushal S. Dave [Dave and Varma, 2010] used semantically related ads. Deepak Agarwal [Agarwal et al., 2010] used existing hierarchical information between ad categories to help predict CTR of new ads. However, these methods cannot be directly applied to image display ads. ..

Background on: Audio Ads Feature Extraction
. [Prockup2015a] the authors designed and implemented a set of deterministic rhythmic descriptors that are tempo-invariant and represent specific elements of the rhythmic attributes. 	


\begin{table*}[]
\centering
\caption{Audio Acoustic Features}
\label{my-label}
\linespread{0.9} %decrease the vertical spacing between lines
\rmfamily 
\begin{tabular}{l|lll|}
\cline{2-4}
 & Feature & Dim & Description \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Timbre}} & TFD & 10 & \begin{tabular}[c]{@{}l@{}}Block Temporal Features and Dynamics - block summary of of each\\ frame's root-mean-square amplitude and zero-crossing rate\end{tabular} \\
\multicolumn{1}{|l|}{} & MFCC & 460 & \begin{tabular}[c]{@{}l@{}}Block MFCCs - capture overall spectral shape - \\ block summary of of each frame\end{tabular} \\
\multicolumn{1}{|l|}{} & DMFCC & 460 & \begin{tabular}[c]{@{}l@{}}Block Delta MFCCs -,capture change in spectral shape - \\ block summary of of each frame\end{tabular} \\
\multicolumn{1}{|l|}{} & MSP & 320 & \begin{tabular}[c]{@{}l@{}}Block Mel-Spectral Patterns - \\ capture patterns in spectral shape\end{tabular} \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Rhythm}} & Tempo & 512 & A primary and secondary estimate of the beats per minute. \\
\multicolumn{1}{|l|}{} & TGLIN & 500 & \begin{tabular}[c]{@{}l@{}}A histogram-like feature that shows emphasis of rhythmic repetition\\ vs a bpm. Each dimension represents a bpm tempo (0-499 BPM)\end{tabular} \\
\multicolumn{1}{|l|}{} & TGR\{B,T,H\} & 13x3 & \begin{tabular}[c]{@{}l@{}}Multi-band Tempogram Ratios for B(A0-A3), T(A3-A6), H(A6-A9). \\ A compact representation of the tempogram at musically important ratios \\ of an estimated tempo.\end{tabular} \\
\multicolumn{1}{|l|}{} & BPDIST\{B,T,H\} & 36x3 & \begin{tabular}[c]{@{}l@{}}Multi-band Beat Profile Distributions for B(A0-A3), T(A3-A6), H(A6-A9). \\ Captures an average snapshot of emphasis of events within the beat.\end{tabular} \\
\multicolumn{1}{|l|}{} & Mellin & 512 & Mellin Scale transform - rhythmic self-similarity among multiple time scales \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Harmony}} & MODE & 1 & Estimate of major of minor mode \\
\multicolumn{1}{|l|}{} & SICH & 18 & Shift-invariant chord histogram - histogram of chords present \\
\multicolumn{1}{|l|}{} & SICHC & 18 & Shift-invariant chord correlations \\
\multicolumn{1}{|l|}{} & SIHPCP & 9 & Shift-Invariant chroma histogram - histogram of notes present \\
\multicolumn{1}{|l|}{} & SIKC & 18 & Shift-invaiant key correlations \\ \hline
\end{tabular}
\end{table*}


Background on using acoustic features for predicting music qualities
 
Background on: (Audio-)Ads Quality Prediction

\section{Problem Definition}
Given  an audio ad, we would like to find the probability that ad is of high quality.

\section{Models}
\subsection{ML based Models}
\subsubsection*{Dimension Reduction and Feature Extraction}
Using  acoustic features on audio files, there is  total number of 2440 variables. Since these variables may be correlated or redundant, we first need to examine some dimension reduction/ feature extraction techniques in order to come up with the underlying  important features. The techniques used in this paper are:
PCA and Kernel PCA, Feature selection based on importance calculated from Tree Classifiers, L1 penalty on Logistic Regression, and L1 penalty on linear SVC, Feature selection based on AUC density 
\subsubsection{ML classification methods}
We will perform the following classification methods on selected features from section above, or on all variables.
Weighted Logistic Regression\\
Random Forest classifier\\
Ada boost + Decision Tree\\
Bagging Classifier + Logistic Regression\\
Support Vector Machines\\
We perform a 10-fold cross validation using each method and record the mean and confidence interval of the AUC of test splits. 
\subsection{NN based Models}
Deep Learning on Acoustic Features \\
Deep Learning on Audio file spectrum \\
Deep Learning on Acoustic + Audio File Spectrum\\
\section{Experimental Study}
\subsection{Datasets}
In advertisement effectiveness, coming with the right labels to define a good/bad audio file is challenging. In this section we will focus on two different type of data with different labels. The first data is collected by a user study in 2016, and the second data defines the labels based on click through rate of the audio ad. Based on this we examine the following datasets in our study.
\begin{itemize}
\item Dataset I: Pandora Ratings 
This data is collected by a study conducted in 2016. 500 audio ads were played on 5 listeners, each listener based on the audio ad could give a rating of ( Positive, Negative, Somewhere in the middle, and Cannot be determined). 
\item Dataset II: Pandora FirstWeek2017
This data consists of 1500 creatives with a value of quality associated to. This value is the fraction of number of clicks over total number of impressions. 
\item Dataset III: Pandora May2017\\
This data consists of 5000 creatives with a value of quality associated to. This value is the fraction of number of clicks over total number of impressions. T
\end{itemize}
Labeling:
To categorize the data as good/bad we need to define meaningful labels for the data provided. Label definition is as follows for each dataset:
Data Set I:

\begin{figure}
\includegraphics[width=.7\linewidth, height=.15\textheight]{Labeling}
\caption{Binary Labels of Dataset II and III based on click through rate}
\label{D23_label}
\end{figure}

\subsection{Experimental Results}
\subsubsection{ML Based Methods}
The results for ML based Method is shown in figure ...

% \begin{figure*}
% \includegraphics[height=1.5in, width=6in]{AUC_methods_D2_L3}
% \caption{A sample black and white graphic
% that needs to span two columns of text.}
% \end{figure*}

\begin{figure*}[ht]
  \centering
  
    \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=.9\linewidth, height=0.1\textheight]{AUC_methods_D1}
    \caption{DataSet I}
  \end{subfigure}  
  
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=.9\linewidth, height=0.1\textheight]{AUC_methods_D2_L3}
    \caption{DataSet II- Labeling III}
  \end{subfigure}

  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=.9\linewidth, height=0.1\textheight]{AUC_methods_D3_L3}
    \caption{DataSet III- Labeling III}
  \end{subfigure}  
  \caption{Test AUC boxplots using 10-fold CV}
  \label{AUC_ML}
\end{figure*}  

\section{Conclusions}
This paragraph will end the body of this sample document.
Remember that you might still have Acknowledgments or
Appendices; brief samples of these
follow.  There is still the Bibliography to deal with; and
we will make a disclaimer about that here: with the exception
of the reference to the \LaTeX\ book, the citations in
this paper are to articles which have nothing to
do with the present subject and are used as
examples only.
%\end{document}  % This is where a 'short' article might terminate


\begin{acks}
  The authors would like to thank ..

\end{acks}


==> model.tex <==
%!TEX root = paper.tex
%
\pv{Assigned: Samaneh, Puya}
\begin{itemize}
\item Acoustic Features (hands crafted) 
\item machine learning (definition of the loss function...), all the features selection methodologies.... 
\item Neural Network (supervised) on spectrogram or features (what are the problems, patches description, sampling, dropout, architecture of CNN, and our network) 
%\item Neural Network (unsupervised) on spectrogram (what are the problems, patches description, sampling, dropout)
\end{itemize}


\subsection{Modeling on Acoustic Features}
\subsubsection*{Dimension Reduction and Feature Extraction}
Using  acoustic features on audio files, there is  total number of 2440 variables. Since these variables may be correlated or redundant, we first need to examine some dimension reduction/ feature extraction techniques in order to come up with the underlying  important features. The techniques used in this paper are:
PCA and Kernel PCA, Feature selection based on importance calculated from Tree Classifiers, L1 penalty on Logistic Regression, and L1 penalty on linear SVC, Feature selection based on AUC density 
\subsubsection{ML classification methods}
We will perform the following classification methods on selected features from section above, or on all variables.
Weighted Logistic Regression\\
Random Forest classifier\\
Ada boost + Decision Tree\\
Bagging Classifier + Logistic Regression\\
Support Vector Machines\\
We perform a 10-fold cross validation using each method and record the mean and confidence interval of the AUC of test splits. 
\subsection{NN based Models}
Deep Learning on Acoustic Features \\
Deep Learning on Audio file spectrum \\
Deep Learning on Acoustic + Audio File Spectrum\\

